Blue Straggler Stars in Globular Clusters: a powerful tool to probe the internal dynamical evolution of stellar systems

This chapter presents an overview of the main observational results obtained to date about Blue Straggler Stars (BSSs) in Galactic Globular Clusters (GCs). The BSS specific frequency, radial distribution, chemical composition and rotational properties are presented and discussed in the framework of using this stellar population as probe of GC internal dynamics. In particular, the shape of the BSS radial distribution has been found to be a powerful tracer of the dynamical age of stellar systems, thus allowing the definition of the first empirical "dynamical clock".

==> common.tex <==
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\newcommand{\gras}[1]{\mbox{\boldmath $#1$}}
\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}          }\hbox{$\frown$}}}$}}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\lsim{\lower.5ex\hbox{\ltsima}}
\def\gsim{\lower.5ex\hbox{\gtsima}}
\def\lapp{\ifmmode\stackrel{<}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}
\def\gapp{\ifmmode\stackrel{>}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}

\def\msol{\,\mathrm{M}_\odot}
\def\media#1{\langle #1\rangle}
\def\kms{~{\rm km~ s}^{-1}}
\def\sigp{\sigma_{\rm P}}


\def\aapr{A\&A Rev. }
\def\apjl{ApJL }
\def\aj{AJ }
\def\apj{ApJ }
\def\pasp{PASP }
\def\spie{SPIE }
\def\apjs{ApJS }
\def\araa{ARAA }
\def\aap{A\&A }
\def\mnras{MNRAS }
\def\nat{Nature }

\newcommand{\lesssim}    {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{<}}}}%
\newcommand{\lsim}       {\lesssim}%
\newcommand{\la}         {\lesssim}% For Springer A&A compliance...
\newcommand{\gtrsim}     {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{>}}}}%
\newcommand{\gsim}       {\gtrsim}%
\newcommand{\ga}         {\gtrsim}%
\newcommand{\sq}         {\mbox{\rlap{\ensuremath{\sqcap}}\ensuremath{\sqcup}}}%
\newcommand{\arcdeg}     {\mbox{\ensuremath{{}^\circ}}}%
\newcommand{\arcmin}     {\mbox{\ensuremath{{}^\prime}}}%
\newcommand{\arcsec}     {\mbox{\ensuremath{{}^{\prime\prime}}}}%

% Journal abbreviations
\def\aj{\rmfamily{AJ~}}           % Astronomical Journal
\def\apj{\rmfamily{ApJ~}}         % Astrophysical Journal
\def\apjl{\rmfamily{ApJ~}}        % Astrophysical Journal, Letters
\def\apjs{\rmfamily{ApJS~}}       % Astrophysical Journal, Supplement
\let\apjlett=\apjl
\let\apjsupp=\apjs
\def\aap{\rmfamily{A\&A~}}        % Astronomy and Astrophysics
\let\astap=\aap
\def\araa{\rmfamily{ARA\&A~}}     % Annual Review of Astronomy and Astrophysics
\def\aapr{\rmfamily{A\&A~Rev.~}}  % Astronomy and Astrophysics Reviews
\def\aaps{\rmfamily{A\&AS~}}      % Astronomy and Astrophysics, Supplement
\def\mnras{\rmfamily{MNRAS~}}     % Monthly Notices of the Royal Astron. Soc.
\def\pasp{\rmfamily{PASP~}}       % Publications of the Astron. Soc. o/t Pacific
\def\apss{\rmfamily{Ap\&SS~}}     % Astrophysics and Space Science
\def\pasj{\rmfamily{PASJ~}}       % Publications of the Astron. Soc. of Japan
\def\pra{\rmfamily{Phys.~Rev.~A~}}% Physical Review A: Atomic, Molecular, and  
                                  %   Optical Physics
\def\prb{\rmfamily{Phys.~Rev.~B~}}% Physical Review B: Condensed Matter and
                                  %   Materials Physics
\def\prc{\rmfamily{Phys.~Rev.~C~}}% Physical Review C: Nuclear Physics
\def\prd{\rmfamily{Phys.~Rev.~D~}}% Physical Review D: Particles, Fields,
                                  %   Gravitation and Cosmology
\def\pre{\rmfamily{Phys.~Rev.~E~}}% Physical Review E: Statistical, Nonlinear,
                                  %   and Soft Matter Physics
\def\rmp{\rmfamily{Rev.~Mod.~Phys.~}}% Reviews of Modern Physics
\def\prl{\rmfamily{Phys.~Rev.~Lett.~}}% Physical Review Letters
\def\nat{\rmfamily{Nature~}}      % Nature
\def\sci{\rmfamily{Science~}}     % Science
\def\skytel{\rmfamily{S\&T~}}     % Sky and Telescope
\def\ao{\rmfamily{Appl.~Opt.~}}   % Applied Optics
\let\applopt=\ao
\def\azh{\rmfamily{AZh~}}         % Astronomicheskii Zhurnal
\def\baas{\rmfamily{BAAS~}}       % Bulletin of the AAS
\def\jrasc{\rmfamily{JRASC~}}     % Journal of the Royal Astron. Soc. of Canada
\def\memras{\rmfamily{MmRAS~}}    % Memoirs of the Royal Astron. Soc.
\def\qjras{\rmfamily{QJRAS~}}     % Quarterly Journal of the Royal Astron. Soc.
\def\solphys{\rmfamily{Sol.~Phys.~}}% Solar Physics
\def\sovast{\rmfamily{Soviet~Ast.~}}% Soviet Astronomy
\def\ssr{\rmfamily{Space~Sci.~Rev.~}}% Space Science Reviews
\def\zap{\rmfamily{ZAp~}}         % Zeitschrift fuer Astrophysik
\def\iauc{\rmfamily{IAU~Circ.~}}  % IAU Cirulars
\let\iaucirc=\iauc
\def\aplett{\rmfamily{Astrophys.~Lett.~}}% Astrophysics Letters
\def\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.~}}% Astrophysics Space Physics
                                  % Research
\def\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands~}}% Bulletin of the 
                                  % Astronomical Institute of the Netherlands
\def\fcp{\rmfamily{Fund.~Cosmic~Phys.~}}% Fundamental Cosmic Physics
\def\gca{\rmfamily{Geochim.~Cosmochim.~Acta~}}% Geochimica Cosmochimica Acta
\def\grl{\rmfamily{Geophys.~Res.~Lett.~}}% Geophysics Research Letters
\def\jcp{\rmfamily{J.~Chem.~Phys.~}}% Journal of Chemical Physics
\def\jgr{\rmfamily{J.~Geophys.~Res.~}}% Journal of Geophysics Research
\def\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.~}} % Journal of Quantitative
                                  % Spectroscopy and Radiative Transfer
\def\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana~}}
                                  % Mem. Societa Astronomica Italiana
\def\nphysa{\rmfamily{Nucl.~Phys.~A~}}% Nuclear Physics A
\def\physrep{\rmfamily{Phys.~Rep.~}}% Physics Reports
\def\physscr{\rmfamily{Phys.~Scr~}}% Physica Scripta
\def\planss{\rmfamily{Planet.~Space~Sci.~}}% Planetary Space Science
\def\procspie{\rmfamily{Proc.~SPIE~}}% Proceedings of the SPIE
\def\aipconf{\rmfamily{AIP~Conf.~Proc.~}}% AIP Conference Proceedings
\def\aspconf{\rmfamily{ASP~Conf.~Ser.~}}% ASP Conference Series
\def\asslconf{\rmfamily{Ap\&SSL~Conf.~Ser.~}}% ASSL Conference Series}
\def\maps{\rmfamily{MAPS~}}       % Meteoritics and Planetary Science

\usepackage{amsmath}
\usepackage{amssymb}

\def\Teff{$T_{\rm eff}$}
\def\Msun{{\rm M}_\odot}
\def\Rsun{{\rm R}_\odot}
\def\kms{\rm km~s$^{-1}$}

\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}                         }\hbox{$\frown$}}}$}}

\newcommand{\msun}{$M_{\odot}$}
\newcommand{\etal}{{\it et al.}}


\newcommand{\half}{{\ensuremath{\textstyle\frac12}}}
\newcommand{\threehalf}{{\ensuremath{\textstyle\frac32}}}
\newcommand{\third}{{\ensuremath{\textstyle\frac13}}}
\newcommand{\quarter}{{\ensuremath{\textstyle\frac14}}}
\newcommand\apgt{\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand\aplt{\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }

\newcommand{\kin}{{\ensuremath K}}
\newcommand{\mbar}{{\ensuremath \langle m\rangle}}
\newcommand{\msun}{{\ensuremath M_\odot}}
\newcommand{\pot}{{\ensuremath U}}
\newcommand{\rvir}{{\ensuremath R_{vir}}}
\newcommand{\rh}{{\ensuremath R_h}}
\newcommand{\rj}{{\ensuremath R_J}}
\newcommand{\rsun}{{\ensuremath R_\odot}}
\newcommand{\tcc}{{\ensuremath t_{cc}}}
\newcommand{\tdis}{{\ensuremath t_{dis}}}
\newcommand{\tdyn}{{\ensuremath t_{dyn}}}
\newcommand{\tr}{{\ensuremath t_r}}
\newcommand{\tenc}{{\ensuremath t_{enc}}}
\newcommand{\trh}{{\ensuremath t_{rh}}}
\newcommand{\trl}{{\ensuremath t_{rl}}}
\newcommand{\tseg}{{\ensuremath t_{seg}}}
\newcommand{\vdisp}{{\ensuremath \langle v^2\rangle}}
\newcommand{\vrms}{{\ensuremath \vdisp^{1/2}}}
\newcommand{\vesc}{{\ensuremath v_{esc}}}
\newcommand{\vinf}{{\ensuremath v_\infty}}

\newcommand{\vv}{{\bf v}}
\newcommand{\vx}{{\bf x}}
\newcommand{\va}{{\bf a}}





